Multiscale Modeling Framework using Element-based Galerkin Methods for Moist Atmospheric Limited-Area Simulations

This paper presents a multiscale modeling framework (MMF) to model moist atmospheric limited-area weather. The MMF resolves large-scale convection using a coarse grid while simultaneously resolving local features through numerous fine local grids and coupling them seamlessly. Both large- and small-scale processes are modeled using the compressible Navier-Stokes equations within the Nonhydrostatic Unified Model of the Atmosphere (NUMA), and they are discretized using a continuous element-based Galerkin method (spectral elements) with high-order basis functions. Consequently, the large-scale and small-scale models share the same dynamical core but have the flexibility to be adjusted individually. The proposed MMF method is tested in 2D and 3D idealized limited-area weather problems involving storm clouds produced by squall line and supercell simulations. The MMF numerical results showed enhanced representation of cloud processes compared to the coarse model.

==> sections/Abstract.tex <==
\section*{Abstract}

This paper presents a multiscale modeling framework (MMF) to model moist atmospheric limited-area weather. The MMF resolves large-scale convection using a coarse grid while simultaneously resolving local features through numerous fine local grids and coupling them seamlessly. Both large- and small-scale processes are modeled using the compressible Navier-Stokes equations within the Nonhydrostatic Unified Model of the Atmosphere (NUMA), and they are discretized using element-based Galerkin methods with high-order basis functions. Consequently, the large-scale and small-scale models share the same dynamical core but have the flexibility to be adjusted individually. The proposed MMF method is tested in 2D and 3D idealized limited-area weather problems involving storm clouds produced by squall line and supercell simulations.

\textit{Keyword:} multiscale modeling framework (MMF), superparameterization, compressible Navier-Stokes equations, precipitation microphysics, element-based Galerkin method, numerical weather prediction.


==> sections/TI.tex <==
\subsection{Implicit-explicit (IMEX) time integration}

We integrate the discretized equation \eqref{eq:governing:matrix} in time using an implicit-explicit (IMEX) time integrator \cite{giraldo2013implicit}. In the IMEX method, the terms responsible for fast waves, such as acoustic and gravity waves, are discretized implicitly, while the other terms for slower advective waves are discretized explicitly. This IMEX strategy enables the use of larger time steps by eliminating the tight CFL restriction due to the fast waves. In this work, we employ the second-order additive Runge-Kutta (ARK2) scheme proposed in \cite{giraldo2013implicit}, which belongs to a family of linear multistage schemes. This time integrator is also used in \cite{giraldo2023performance} by referring to ARK(2,3,2)b. We solve the linear system that arises from the implicit part of the IMEX formulation using the iterative Krylov subspace GMRES \cite[pg. 266]{trefethen1997} in a matrix-free fashion. While the MMF method offers flexibility in selecting different time integrators for LSP and SSP models, we choose to use the same time integrators for both the models in MMF simulations in this work. In future work, we will explore the use of different time integrators and orders of accuracy for the SSP models. 


